CLASH: Three Strongly Lensed Images of a Candidate z ~ 11 Galaxy

We present a candidate for the most distant galaxy known to date with a photometric redshift z = 10.7 +0.6 / -0.4 (95% confidence limits; with z < 9.5 galaxies of known types ruled out at 7.2-sigma). This J-dropout Lyman Break Galaxy, named MACS0647-JD, was discovered as part of the Cluster Lensing and Supernova survey with Hubble (CLASH). We observe three magnified images of this galaxy due to strong gravitational lensing by the galaxy cluster MACSJ0647.7+7015 at z = 0.591. The images are magnified by factors of ~8, 7, and 2, with the brighter two observed at ~26th magnitude AB (~0.15 uJy) in the WFC3/IR F160W filter (~1.4 - 1.7 um) where they are detected at >~ 12-sigma. All three images are also confidently detected at >~ 6-sigma in F140W (~1.2 - 1.6 um), dropping out of detection from 15 lower wavelength HST filters (~0.2 - 1.4 um), and lacking bright detections in Spitzer/IRAC 3.6um and 4.5um imaging (~3.2 - 5.0 um). We rule out a broad range of possible lower redshift interlopers, including some previously published as high redshift candidates. Our high redshift conclusion is more conservative than if we had neglected a Bayesian photometric redshift prior. Given CLASH observations of 17 high mass clusters to date, our discoveries of MACS0647-JD at z ~ 10.8 and MACS1149-JD1 at z ~ 9.6 are consistent with a lensed luminosity function extrapolated from lower redshifts. This would suggest that low luminosity galaxies could have reionized the universe. However given the significant uncertainties based on only two galaxies, we cannot yet rule out the sharp drop off in number counts at z >~ 10 suggested by field searches.

==> figs2-6.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HST images

\begin{figure*}
%\centerline{\includegraphics[width = 0.95\textwidth]{figs/JD3stamps.png}}
\centerline{HSTstamps.png}
%~/CLASH/data/m0647/images/stamps/stampmontageheat.py
%\captionsetup{labelsep=pipe}
\caption{
\label{fig:HST}
The three images of \JD\ as observed in various filters with HST.
%
The leftmost panels show the summed 11-hour (17-orbit)
exposures obtained
in 8 filters spanning 0.4--0.9\um\ with the Advanced Camera for Surveys.
%
The five middle columns show observations with the Wide Field Camera 3 IR channel
in F105W, F110W, F125W, F140W, and F160W,
all shown with the same linear scale in electrons per second.
%
The F125W images were obtained at a single roll angle,
and a small region near JD2 was affected by persistence due to a moderately bright star in our parallel observations immediately prior
(see also Fig.~\ref{fig:timeimages}).
%
The right panels zoom in by a factor of 2 to show F110W+F140W+F160W color images scaled linearly between 0 and 0.1 \uJy.
% ~/CLASH/data/m0647/images/stamps/colorimage.py
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series fluxes
\begin{figure*}
\centerline{fluxseriesnew.png}
%\captionsetup{labelsep=pipe}
\caption{
\label{fig:timeflux}
Flux measurements in the individual epochs observed over a period of 56 days.
Filters are colored F160W (red), F140W (yellow), F125W (green), and F110W (blue)
as both individual data points and solid bands as determined for the summed observations.
%
The F110W exposures obtained in the second epoch (visit A9)
were found to have significantly elevated and non-Poissonian backgrounds
due to Earthshine (\S\ref{sec:HSTphot}).
These were excluded in our analysis; we adopted the F110W fluxes measured in the first epoch (visit A2).
%or reflections from the sunlit Earth (see \S\ref{sec:HSTphot}).
%within 30 degrees of the daytime Earth horizon (limb).
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HST SED

\begin{figure*}
%\centerline{\includegraphics[width = \textwidth]{figs/Khoised.png}}
%\centerline{\includegraphics[width = \textwidth]{figs/KhoiNamased.png}}
%\centerline{\includegraphics[width = \textwidth]{figs/sed_JD_HST.png}}
\centerline{sed_JD_HST_new.png}
%\captionsetup{labelsep=pipe}
\caption{
\label{fig:HSTsed}
Observed HST photometry (filled circles and triangles)
plotted against the expected fluxes (open blue squares)
from a young starburst galaxy spectrum (gray line) redshifted to $z \sim 11$.
%
HST filter transmission curves are plotted in the upper panel,
normalized to their maxima,
and with black dots indicating the effective ``pivot'' wavelengths.
%
Photometry of the \Jdrops\ observed through these filters (Table \ref{tab:cat})
is plotted as the larger
circles and triangles for positive and negative observed fluxes, respectively,
with 1-$\sigma$ error bars.
%
For some points, horizontal ``error bars'' are plotted to reiterate the filter widths.
%
The gray line is a model spectrum of a young starburst at $z = 11.0$, the best fit to the summed photometry.
%$z = 11.03$.
%
The integrals of this spectrum through our filters
give the model predicted fluxes plotted as blue squares.
Other galaxy types at $z \sim 11$ yield similar predicted HST fluxes,
as the shape of the spectrum cannot be constrained by the HST photometry alone.
Redshifted Lyman-$\alpha$ at $0.1216\mu$m$(1+z) \sim 1.46\mu$m is indicated by the vertical dashed line.
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series images F140W & F160W
\begin{figure*}
\centerline{timeseries.png}
%\captionsetup{labelsep=pipe}
\caption{
\label{fig:timeimages}
\JD\ as observed in each of the individual epochs of F160W and F140W obtained over a 56-day period.
%
These observations were obtained at two different telescope roll angles
which alternate between the stamps shown here.
A small region of the WFC3/IR images in our first roll angle
was affected by persistence due to a moderately bright star in our parallel observations immediately prior.
These pixels happen to fall within $1''$ of JD2 at that roll angle
(marked in gray here and flagged as unreliable).
Excluding this roll angle for JD2 does not significantly affect the derived photometry.
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series centroids
\begin{figure*}
\centerline{timeseriesxy.png}
}
%\captionsetup{labelsep=pipe}
\caption{
\label{fig:timexy}
Relative centroid measurements for the detections in F160W (red) and F140W (yellow)
in individual epochs (circles) and summed observations (squares).
Centroids measured in the summed NIR images are also plotted as gray diamonds.
The offsets are generally less than one of our drizzled pixels ($0.065''$),
roughly half the native WFC3/IR pixel size ($\sim$0.13$''$).
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%


